Modeling an Asynchronous Circuit Dedicated to the Protection Against Physical Attacks

Asynchronous circuits have several advantages for security applications, in particular their good resistance to attacks. In this paper, we report on experiments with modeling, at various abstraction levels, a patented asynchronous circuit for detecting physical attacks, such as cutting wires or producing short-circuits.

==> eptcsdata.tex <==
\providecommand{\firstpage}{200}
\providecommand{\publicationstatus}{A. Fehnker and H. Garavel (Eds.):\\
Models for Formal Analysis of Real Systems (MARS 2020)\\
EPTCS 316, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.316.8}{10.4204/EPTCS.316.8}}


==> protocol_cycle_fig.tex <==
\begin{picture}(0,0)%
\includegraphics{protocol_cycle}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2730,1245)(436,-751)
\end{picture}%


==> sequencer_fig.tex <==
\begin{picture}(0,0)%
\includegraphics{sequencer}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(6865,1664)(-844,-1118)
\end{picture}%


==> serial_shield_fig.tex <==
\begin{picture}(0,0)%
\includegraphics{serial_shield}%
\end{picture}%
\setlength{\unitlength}{3729sp}%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(7041,719)(429,-758)
\end{picture}%


==> short_circuit_fig.tex <==
\begin{picture}(0,0)%
\includegraphics{short_circuit}%
\end{picture}%
\setlength{\unitlength}{3315sp}%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5952,719)(-21,-758)
\end{picture}%

